Within the Dynamic Context: Inertia-aware 3D Human Modeling with Pose Sequence

Neural rendering techniques have significantly advanced 3D human body modeling. However, previous approaches often overlook dynamics induced by factors such as motion inertia, leading to challenges in scenarios like abrupt stops after rotation, where the pose remains static while the appearance changes. This limitation arises from reliance on a single pose as conditional input, resulting in ambiguity in mapping one pose to multiple appearances. In this study, we elucidate that variations in human appearance depend not only on the current frame's pose condition but also on past pose states. Therefore, we introduce Dyco, a novel method utilizing the delta pose sequence representation for non-rigid deformations and canonical space to effectively model temporal appearance variations. To prevent a decrease in the model's generalization ability to novel poses, we further propose low-dimensional global context to reduce unnecessary inter-body part dependencies and a quantization operation to mitigate overfitting of the delta pose sequence by the model. To validate the effectiveness of our approach, we collected a novel dataset named I3D-Human, with a focus on capturing temporal changes in clothing appearance under approximate poses. Through extensive experiments on both I3D-Human and existing datasets, our approach demonstrates superior qualitative and quantitative performance. In addition, our inertia-aware 3D human method can unprecedentedly simulate appearance changes caused by inertia at different velocities.

==> sections/Results_of_exps.tex <==
\section{Supplementary}


\setlength\tabcolsep{.7em}
\begin{table}[h]
\centering
\caption{Per-subject results on our data. }
\resizebox{\textwidth}{!}{
\begin{tabular}{clcccccccc}
\toprule
\multirow{2}{*}{Subject} &\multirow{2}{*}{Method} & \multicolumn{4}{c}{Novel View} & \multicolumn{4}{c}{Novel Pose} \\
 \cmidrule(lr){3-6} \cmidrule(lr){7-10}
  &  & PSNR & SSIM & LPIPS & New-Metric & PSNR & SSIM & LPIPS & New-Metric \\
\midrule 
xianpei-2&NeuralBody&29.54 & 0.9693 & 51.16 & - & 27.81 & 0.9622 & 57.31 & - \\
xianpei-legswing&NeuralBody&31.08 & 0.9729 & 43.39 & - & 29.64 & 0.9675 & 49.45 & - \\
lingyi-0&NeuralBody&27.82 & 0.9632 & 70.10 & - & 25.48 & 0.9499 & 81.19 & - \\
yuchen-1&NeuralBody&32.07 & 0.9682 & 69.19 & - & 31.28 & 0.9640 & 72.12 & - \\
Average-4 subs&NeuralBody\yutong&30.33 & 0.9681 & 60.89 & - & 28.80 & 0.9604 & 67.59 & - \\
xianpei-2&AniSDF&28.40 & 0.9684 & 52.57 & - & 27.58 & 0.9642 & 56.01 & - \\
xianpei-legswing&AniSDF&29.24 & 0.9675 & 49.59 & - & 28.63 & 0.9655 & 52.10 & - \\
lingyi-0&AniSDF&27.35 & 0.9650 & 64.79 & - & 26.07 & 0.9578 & 70.75 & - \\
yuchen-1&AniSDF&31.80 & 0.9671 & 68.80 & - & 31.08 & 0.9651 & 69.84 & - \\
Average-4 subs&AniSDF&29.20 & 0.9670 & 58.94 & - & 28.34 & 0.9632 & 62.18 & - \\
\midrule

xianpei-2&TPAMI-AniNeRF&28.35 & 0.9674 & 55.81 & - & 27.50 & 0.9634 & 59.10 & - \\
xianpei-legswing&TPAMI-AniNeRF&29.69 & 0.9674 & 52.66 & - & 29.19 & 0.9670 & 52.79 & - \\
lingyi-0&TPAMI-AniNeRF&27.32 & 0.9640 & 69.03 & - & 26.21 & 0.9568 & 76.14 & - \\
yuchen-1&TPAMI-AniNeRF&31.80 & 0.9662 & 70.32 & - & 31.00 & 0.9640 & 71.36 & - \\
Average-4 subs&TPAMI-AniNeRF&29.29 & 0.9662 & 61.95 & - & 28.48 & 0.9628 & 64.85 & - \\
\midrule
&HumanNeRF~\cite{weng2022humannerf}& - & - & - & -  &  -  & - & - & - \\
&MonoHuman~\cite{yu2023monohuman} & - & - & - & -  &  -  & - & - & - \\
\midrule
xianpei-2&3dgs-avatar&29.58 & 0.9705 & 35.00 & - & 28.31 & 0.9663 & 39.85 & - \\
xianpei-legswing&3dgs-avatar&30.79 & 0.9719 & 34.10 & - & 30.25 & 0.9704 & 34.39 & - \\
lingyi-0&3dgs-avatar&29.53 & 0.9710 & 43.47 & - & 26.38 & 0.9581 & 55.73 & - \\
yuchen-1&3dgs-avatar&32.58 & 0.9713 & 46.37 & - & 31.90 & 0.9683 & 48.44 & - \\
% xianpei-sleeve&3dgs-avatar&26.71 & 0.9628 & 54.19 & - & 25.91 & 0.9571 & 55.47 & - \\
% Average-5 subs&3dgs-avatar&29.84 & 0.9695 & 42.63 & - & 28.55 & 0.9640 & 46.78 & - \\
Average-4 subs&3dgs-avatar&30.62 & 0.9712 & 39.74 & - & 29.21 & 0.9658 & 44.61 & - \\

\midrule
xianpei-2&ours&31.31 & 0.9747 & 29.66 & 20.51 & 30.34 & 0.9713 & 34.41 & 18.01 \\
xianpei-legswing&ours&31.20 & 0.9731 & 32.67 & - & 30.45 & 0.9710 & 33.19 & - \\
lingyi-0&ours&29.26 & 0.9716 & 38.02 & - & 27.15 & 0.9617 & 49.07 & - \\
yuchen-1&ours&32.57 & 0.9733 & 40.60 & - & 31.77 & 0.9694 & 45.17 & - \\
Average-4 subs&ours&31.09 & 0.9732 & 35.24 & - & 29.93 & 0.9684 & 40.46 & - \\
                     \bottomrule
\end{tabular}
}
\label{table:Results_PJMoCap_PerSubject}
\end{table}


\setlength\tabcolsep{.7em}
\begin{table}[h]
\centering
\caption{Per-subject results on ZJU-MoCap. }
\resizebox{\textwidth}{!}{
\begin{tabular}{clcccccccc}
\toprule
\multirow{2}{*}{Subject} &\multirow{2}{*}{Method} & \multicolumn{4}{c}{Novel View} & \multicolumn{4}{c}{Novel Pose} \\
 \cmidrule(lr){3-6} \cmidrule(lr){7-10}
  &  & PSNR & SSIM & LPIPS & New-Metric & PSNR & SSIM & LPIPS & New-Metric \\

\midrule
% TODO  Neuralbody eval_whole_image=True
%According to https://github.com/ChenYutongTHU/neuralbody/blob/master/supplementary_material.md
313&NeuralBody&35.21 & 0.9857 & 31.29 & - & 29.06 & 0.9641 & 52.23 & - \\
315&NeuralBody&32.91 & 0.9875 & 28.27 & - & 25.69 & 0.9574 & 51.95 & - \\
377&NeuralBody&33.75 & 0.9851 & 27.91 & - & 30.49 & 0.9768 & 35.02 & - \\
386&NeuralBody&36.00 & 0.9845 & 28.66 & - & 33.03 & 0.9745 & 43.95 & - \\
387&NeuralBody&31.32 & 0.9747 & 44.73 & - & 27.67 & 0.9615 & 53.97 & - \\
390&NeuralBody&30.15 & 0.9633 & 54.03 & - & 31.89 & 0.9713 & 43.29 & - \\ /Error
392&NeuralBody&35.65 & 0.9841 & 33.91 & - & 31.43 & 0.9708 & 48.72 & - \\
393&NeuralBody&33.16 & 0.9788 & 39.22 & - & 28.33 & 0.9601 & 54.76 & - \\
394&NeuralBody&34.19 & 0.9799 & 36.28 & - & 29.51 & 0.9613 & 54.54 & - \\
Average-9 subs&NeuralBody&33.59 & 0.9804 & 36.03 & - & 29.68 & 0.9664 & 48.71 & - \\
\midrule
313&TPAMI-AniNeRF&32.41 & 0.9758 & 40.55 & - & 27.75 & 0.9580 & 53.99 & - \\
315&TPAMI-AniNeRF&29.54 & 0.9749 & 47.71 & - & 25.61 & 0.9550 & 59.93 & - \\
377&TPAMI-AniNeRF&32.63 & 0.9813 & 37.49 & - & 31.30 & 0.9787 & 38.24 & - \\
386&TPAMI-AniNeRF&35.38 & 0.9812 & 39.77 & - & 33.47 & 0.9765 & 43.44 & - \\
387&TPAMI-AniNeRF&30.58 & 0.9684 & 57.94 & - & 28.94 & 0.9641 & 57.73 & - \\
390&TPAMI-AniNeRF&30.03 & 0.9654 & 56.96 & - & 32.02 & 0.9724 & 49.62 & - \\
392&TPAMI-AniNeRF&34.23 & 0.9786 & 48.47 & - & 31.18 & 0.9704 & 54.70 & - \\
393&TPAMI-AniNeRF&32.16 & 0.9732 & 53.44 & - & 28.58 & 0.9607 & 62.75 & - \\
394&TPAMI-AniNeRF&33.61 & 0.9765 & 45.43 & - & 29.86 & 0.9643 & 53.08 & - \\
Average-9 subs&TPAMI-AniNeRF&32.69 & 0.9764 & 45.91 & - & 29.71 & 0.9662 & 53.28 & - \\
\midrule
313&AniSDF&32.84 & 0.9788 & 30.86 & - & 27.63 & 0.9586 & 45.83 & - \\
315&AniSDF&29.78 & 0.9782 & 37.67 & - & 25.44 & 0.9565 & 48.83 & - \\
377&AniSDF&32.65 & 0.9825 & 33.22 & - & 31.07 & 0.9794 & 34.47 & - \\
386&AniSDF&34.73 & 0.9814 & 36.33 & - & 33.41 & 0.9766 & 39.10 & - \\
387&AniSDF&30.49 & 0.9709 & 49.93 & - & 28.74 & 0.9661 & 50.15 & - \\
390&AniSDF&33.39 & 0.9789 & 37.33 & - & 30.94 & 0.9703 & 47.05 & - \\
%390&AniSDF&30.01 & 0.9677 & 48.07 & - & 31.76 & 0.9740 & 42.85 & - \\
392&AniSDF&33.80 & 0.9785 & 44.84 & - & 30.67 & 0.9711 & 49.93 & - \\
393&AniSDF&31.82 & 0.9750 & 45.53 & - & 28.09 & 0.9626 & 53.03 & - \\
394&AniSDF&33.36 & 0.9774 & 39.23 & - & 29.36 & 0.9645 & 46.49 & - \\
Average-9 subs&AniSDF&32.54 & 0.9779 & 39.44 & - & 29.48 & 0.9673 & 46.10 & - \\
%Average-9 subs&AniSDF&32.16 & 0.9767 & 40.63 & - & 29.58 & 0.9677 & 45.63 & - \\

&HumanNeRF~\cite{weng2022humannerf}& - & - & - & -  &  -  & - & - & - \\
&MonoHuman~\cite{yu2023monohuman} & - & - & - & -  &  -  & - & - & - \\
\midrule

313&3dgs-avatar&35.23 & 0.9868 & 17.85 & - & 28.76 & 0.9654 & 33.78 & - \\
315&3dgs-avatar&29.57 & 0.9796 & 20.96 & - & 25.92 & 0.9621 & 30.77 & - \\
392&3dgs-avatar&33.89 & 0.9802 & 24.53 & - & 31.22 & 0.9734 & 30.37 & - \\
394&3dgs-avatar&33.30 & 0.9767 & 24.08 & - & 30.37 & 0.9679 & 30.70 & - \\
393&3dgs-avatar&31.50 & 0.9734 & 27.64 & - & 29.20 & 0.9657 & 33.77 & - \\
377&3dgs-avatar&32.40 & 0.9829 & 18.31 & - & 31.41 & 0.9805 & 20.14 & - \\
386&3dgs-avatar&35.30 & 0.9823 & 23.69 & - & 33.64 & 0.9774 & 27.47 & - \\
387&3dgs-avatar&30.61 & 0.9721 & 30.02 & - & 28.93 & 0.9674 & 31.11 & - \\
390&3dgs-avatar&33.49 & 0.9778 & 26.79 & - & 30.65 & 0.9693 & 33.64 & - \\
Average-9 subs&3dgs-avatar&32.81 & 0.9791 & 23.76 & - & 30.01 & 0.9699 & 30.20 & - \\

313&humannerf&33.41 & 0.9845 & 17.56 & - & 28.49 & 0.9622 & 35.79 & - \\
313&ours-A100x4&34.17 & 0.9838 & 19.66 & - & 28.03 & 0.9589 & 42.21 & - \\
313&ours-3090x1&34.28 & 0.9847 & 17.96 & - & 27.97 & 0.9590 & 41.13 & - \\
313&yifn-3090x1&34.47 & 0.9850 & 18.19 & - & 28.20 & 0.9613 & 38.90 & - \\


315&ours-A100x4&29.80 & 0.9818 & 15.80 & - & 25.30 & 0.9584 & 34.82 & - \\
315&ours-3090x1&29.82 & 0.9818 & 15.92 & - & 25.34 & 0.9590 & 33.88 & - \\
315&yifn-3090x1&29.83 & 0.9820 & 15.63 & - & 25.36 & 0.9585 & 34.24 & - \\
315&humannerf&29.11 & 0.9803 & 17.71 & - & 25.27 & 0.9586 & 32.61& - \\
386&humannerf&34.85 & 0.9823 & 21.55 & - & 33.57 & 0.9765 & 27.76 & - \\
386&ours-3090x4&35.56 & 0.9831 & 21.34 & - & 33.04 & 0.9753 & 28.65 & - \\
386&ours-3090x1r&35.43 & 0.9829 & 20.81 & - & 33.02 & 0.9755 & 28.26 & - \\
386&yifn-3090x1&35.53 & 0.9831 & 20.92 & - & 33.48 & 0.9764 & 28.16 & - \\


387&ours-3090x1&30.61 & 0.9737 & 25.68 & - & 28.64 & 0.9665 & 30.63 & - \\
387&yifn-3090x1&30.58 & 0.9737 & 25.23 & - & 28.74 & 0.9669 & 30.25 & - \\
387&humannerf&30.01 & 0.9712 & 29.42 & - & 28.75 & 0.9667 & 31.55 & - \\

390&humannerf&32.86 & 0.9779 & 24.60 & - & 30.40 & 0.9677 & 34.91 & - \\
390&ours-3090x4&33.43 & 0.9795 & 22.92 & - & 30.46 & 0.9684 & 34.04 & - \\
390&ours-3090x1&33.41 & 0.9791 & 23.12 & - & 30.63 & 0.9686 & 33.59 & - \\
390&yifn-3090x1&33.44 & 0.9798 & 22.54 & - & 30.52 & 0.9687 & 34.20 & - \\

377&ours-3090x1&32.64 & 0.9839 & 15.72 & - & 31.14 & 0.9802 & 18.69 & - \\
377&yifn-3090x1&32.55 & 0.9835 & 16.49 & - & 31.31 & 0.9805 & 19.29 & - \\
377&ours-3090x4&32.65 & 0.9838 & 16.05 & - & 31.03 & 0.9800 & 18.93 & - \\
377&humannerf&32.26 & 0.9826 & 17.87 & - & 31.04& 0.9800 & 20.01 & - \\

392&humannerf&33.10 & 0.9789 & 23.03 & - & 30.76 & 0.9718 & 30.29 & - \\
392&ours-3090x1&34.36 & 0.9816 & 19.75 & - & 31.04 & 0.9724 & 29.99 & - \\
392&yifn-3090x1&34.11 & 0.9809 & 20.42 & - & 31.20 & 0.9725 & 29.92 & - \\
392&ours-3090x4&34.28 & 0.9815 & 19.97 & - & 31.19 & 0.9728 & 29.52 & - \\


393&ours-3090x4&31.67 & 0.9741 & 23.58 & - & 28.63 & 0.9627 & 34.49 & - \\
393&ours-3090x1&31.75 & 0.9742 & 23.95 & - & 28.80 & 0.9630 & 34.23 & - \\
393&yifn-3090x1&31.71 & 0.9743 & 23.55 & - & 28.91 & 0.9638 & 34.26 & - \\
393&humannerf&30.76 & 0.9718 & 26.05 & - &  28.72  & 0.9625 & 34.35  & -\\
394&ours-3090x4&33.57 & 0.9777 & 19.72 & - & 29.72 & 0.9644 & 31.94 & - \\
394&ours-3090x1&33.59 & 0.9779 & 19.65 & - & 29.71 & 0.9648 & 31.62 & - \\
394&yifn-3090x1&33.54 & 0.9775 & 19.95 & - & 29.71 & 0.9643 & 31.80 & - \\
394&humannerf&32.80 & 0.9756 & 22.88 & - & 29.59 & 0.9641 & 32.79 & - \\
 \bottomrule
\end{tabular}}
\label{table:Results_ZJU-MoCap_PerSubject}
\end{table}


==> sections/yutong_notes.tex <==
\section{Yutong's Notes}


\subsection{Command}


Some command for abbreviation.

For example: \eg, blala
\begin{verbatim}
    \eg, blala
\end{verbatim}

That is: \ie, ydayda
\begin{verbatim}
    \ie, ydayda
\end{verbatim}

and so on: A, B and C, \etc should blabla.
\begin{verbatim}
    A, B and C, \etc should blabla.
    ydayda A, B, C, \etc
\end{verbatim}

and others: by Zeus \etal.
\begin{verbatim}
     parties'', by Zeus \etal.
\end{verbatim}

Reference like this (\cref{sec:introduction}) or \Cref{sec:introduction} is the introduction.
  (\ie, for that is. \etc, for ...).

It is also possible to refer to multiple targets as once, \eg~to \cref{fig:example,fig:short-a}.
    
please refrain from using any \LaTeX{} or \TeX{} command that modifies the layout settings of the template (\eg, \verb+\textheight+, \verb+\vspace+, \verb+\baselinestretch+, \etc). Such manual layout adjustments should be limited to very exceptional cases. 

Papers with more than 14 pages (excluding references) will be rejected without review.


\emph{Cite} like this~\cite{Anonymous24b}''.

6\:pt \checkmark 
6 pt $\times$

$\sim$2\:mm \checkmark 
$\sim$2 mm $\times$

\url{https://doi.org/10.1063/1.2811173}.

Distinguish between \etc and \etal.  

"Et cetera" is a Latin phrase that translates to "and the rest" or "and so forth" in English. 

 "Et al." is an abbreviation for the Latin phrase "et alia" (masculine), "et alii" (masculine plural), or "et aliae" (feminine plural), which all mean "and others." It is used to refer to additional authors or contributors when citing a source. It is often used in academic citations to avoid listing all the authors in a long list. 
\begin{itemize}
    \item Smith \etal (2020) conducted a comprehensive study on climate change.
    \item please refrain from using any \LaTeX{} or \TeX{} command that modifies the layout settings of the template (\eg, \verb+\textheight+, \verb+\vspace+, \verb+\baselinestretch+, \etc).
    \item The numbers accorded to lemmas, propositions, and theorems, \etc should appear in consecutive order, starting with Lemma 1. 
    \item How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.
    \item The store sells various fruits such as apples, oranges, bananas, etc.
\end{itemize}

Headings should be capitalized (\ie, {\bf nouns, verbs, and all other words except articles, prepositions, and conjunctions should be set with an initial capital}) and should, with the exception of the title, be aligned to the left.
Only the first two levels of section headings should be numbered, as shown in \cref{tab:headings}.
The respective font sizes are also given in \cref{tab:headings}. 

\subsection{Table}
\begin{table}[tb]
  \caption{Font sizes of headings. 
    Table captions should always be positioned \emph{above} the tables.
  }
  \label{tab:headings}
  \centering
  \begin{tabular}{@{}lll@{}}
    \toprule
    Heading level & Example & Font size and style\\
    \midrule
    Title (centered)  & {\Large\bf Lecture Notes \dots} & 14 point, bold\\
    1st-level heading & {\large\bf 1 Introduction} & 12 point, bold\\
    2nd-level heading & {\bf 2.1 Printing Area} & 10 point, bold\\
    3rd-level heading & {\bf Headings.} Text follows \dots & 10 point, bold\\
    4th-level heading & {\it Remark.} Text follows \dots & 10 point, italic\\
  \bottomrule
  \end{tabular}
\end{table}



\subsection{Figures}
\label{sect:figures}
Us the package \texttt{graphicx}.

It is essential that all illustrations are clear and legible. 
{\it Vector graphics (rather than rasterized images) should be used for diagrams and schemas whenever possible. }

Line drawings are to have a resolution of at least 800 dpi (preferably 1200 dpi).
Grids and details within figures must be clearly legible and may not be written one on top of the other. 
The lettering in figures should not use font sizes smaller than 6\:pt ($\sim$2\:mm character height). 

Figures should be numbered and should have a caption, which should always be positioned \emph{under} the figures.

If they are short, they are centered between the margins (\cf \cref{fig:short}). 
Longer captions, covering more than one line, are justified (\cref{fig:example} shows an example). 
Captions that do not constitute a full sentence, do not have a period.


\begin{figure}[tb]
  \centering
  \includegraphics[height=6.5cm]{eijkel2}
  \caption{One kernel at $x_s$ (\emph{dotted kernel}) or two kernels at $x_i$ and $x_j$ (\emph{left and right}) lead to the same summed estimate at $x_s$.
    This shows a figure consisting of different types of lines.
    {\bf Elements of the figure described in the caption should be set in italics, in parentheses}, as shown in this sample caption. 
    The last sentence of a figure caption should generally end with a full stop, except when the caption is not a full sentence.
  }
  \label{fig:example}
\end{figure}

\begin{figure}[tb]
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Centered, short example caption}
  \label{fig:short}
\end{figure}

If possible (\eg, if you use \LaTeX) please define figures as floating objects. 
\LaTeX{} users, please avoid using the location parameter ``h'' for ``here''.  In LaTeX, a float is an object that is placed within a document but is allowed to "float" to a different location based on certain formatting rules. 

If you have to insert a pagebreak before a figure, please ensure that the previous page is completely filled. 

\subsection{Formulas}
Displayed equations or formulas are centered and set on a separate line (with an extra line or half line space above and below). 
Equations should be numbered for reference. 
The numbers should be consecutive within the contribution, with numbers enclosed in parentheses and set on the right margin.
For example,
\begin{align}
  \psi (u) & = \int_{0}^{T} \left[\frac{1}{2}
  \left(\Lambda_{0}^{-1} u,u\right) + N^{\ast} (-u)\right] \text{d}t \; \\
& = 0
\end{align}
and 
\begin{equation}
  E = m\cdot c^2.
  \label{eq:important}
\end{equation}
Please do not include section counters in the numbering.
\subsection{Footnotes.}

The superscript numeral used to refer to a footnote appears in the text either directly after the word to be discussed or -- in relation to a phrase or a sentence -- following the punctuation mark (comma, semicolon, or period).%
\footnote{The footnote numeral is set flush left and the text follows with the usual word spacing. 
  Second and subsequent lines are indented. 
}

\subsection{Program Code}
Program listings or program commands in the text are normally set in typewriter font (\eg, \texttt{printf("Hello world!\textbackslash{}n");}).

\subsection{Citations}
Arabic numbers are used for citation, which is sequential either by order of citation or by alphabetical order of the references, depending on which sequence is used in the list of references. 
The reference numbers are given in brackets and are not superscript.
Please observe the following guidelines:
\begin{itemize}
\item Single citation: \cite{Anonymous24}
\item Multiple citation: \cite{Alpher02,Alpher03,Alpher05,Anonymous24b,Anonymous24}. 
  The numbers should be listed in numerical order.
  If you use the template as advised, this will be taken care of automatically.
\item If an author's name is used in the text: Alpher \cite{Alpher02} was the first \ldots
\end{itemize}

The \LaTeX{} template already takes care of that through the use of the \texttt{splncs04.bst} Bib\TeX{} style file.
Springer strongly encourages you to include DOIs (Digital Object Identifiers) in your references (\cf \cite{ECCV2022}). 
The DOI is a unique code allotted by the publisher to each online paper or journal article. 
It provides a stable way of finding published papers and their metadata. 

\subsection{Miscellaneous}
Compare the following:
\begin{center}
  \begin{tabular}{ll}
    \verb'$conf_a$'          & $\qquad conf_a$ \\
    \verb'$\mathit{conf}_a$' & $\qquad \mathit{conf}_a$
  \end{tabular}
\end{center}
See The \TeX book, p.\ 165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, \emph{e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', 
shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et\hskip 0.1em}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, {\bf use it only when there are three or more authors.}
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is \emph{incorrect}: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.


==> tables/sota_zju.tex <==
\setlength\tabcolsep{.7em}
\begin{table}[h!]
\centering
\caption{ \textbf{Comparison with state-of-the-arts on ZJU-MoCap}: The scores are averaged over the 9 sequences. Dyco achieves comparable results with state-of-the-arts, preserving the ability of modeling tightly-clothed humans in slow and gradual motion.  $\textrm{LPIPS}^*=\textrm{LPIPS}\times10^3$}

% \footnote{Their original papers compute PSNR and SSIM within a bounding box encompassing the subject. To ensure consistency of the comparison, we re-evaluate their released models on the entire image and report the scores here. }


\resizebox{\textwidth}{!}{
% \begin{tabular}{lcccccc}
% \toprule
%  \multirow{2}{*}{Method} & \multicolumn{3}{c}{Novel View} & \multicolumn{3}{c}{Novel Pose} \\
%  \cmidrule(lr){2-4} \cmidrule(lr){5-7}
%     & PSNR & SSIM & $\textrm{LPIPS}^*$ & PSNR & SSIM & $\textrm{LPIPS}^*$  \\

\begin{tabular}{lcccccccc}
\toprule
 \multirow{2}{*}{Method} & \multicolumn{4}{c}{Novel View} & \multicolumn{4}{c}{Novel Pose} \\
 \cmidrule(lr){2-5} \cmidrule(lr){6-9}
    & PSNR$\uparrow$ & SSIM$\uparrow$ & $\textrm{LPIPS}^*\downarrow$ & DME$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & $\textrm{LPIPS}^*\downarrow$ & DME$\downarrow$ \\
    
\midrule   
NeuralBody~\cite{peng2023implicit}&\textbf{33.59} & \textbf{0.9804 } & 36.03 &\textbf{5.02}& 29.68 & 0.9656 & 49.70 &7.22 \\
AniNeRF~\cite{peng2024animatable}&32.28 & 0.9750 & 47.53 & 5.44 & 29.86 & 0.9667 & 52.61 & 6.91 \\
AniSDF~\cite{peng2024animatable}&32.16 & 0.9767 & 40.63 & 5.60 & 29.58 & 0.9677 & 45.63 & 6.96 \\
HumanNeRF~\cite{weng2022humannerf}& 32.13 & 0.9783 & 22.30 &5.78&  29.62 & 0.9678 & 31.11 &7.43\\
3DGS-Avatar~\cite{qian2023_3dgsavatar} &32.81 & 0.9791 & 23.76 &5.47& \textbf{30.01} & \textbf{0.9699} &\textbf{30.20} &\textbf{6.98}\\
Dyco (Ours) & 32.86 & 0.9790 &\textbf{20.03} &5.50&  29.70 & 0.9667 & 31.09&7.02 \\
                     \bottomrule
\end{tabular}
}
\label{table:sota_zju}
\vspace{-4mm}
\end{table}


